Towards Data-Enabled Physical Activity Planning: An Exploratory Study of HCP Perspectives On The Integration Of Patient-Generated Health Data

Physical activity planning is an essential part of cardiovascular rehabilitation. Through a two-part formative design exploration, we investigated integrating patient-generated health data (PGHD) into clinical workflows supporting shared decision-making (SDM) in physical activity planning. In part one, during a two-week situated study, to reduce risk of working with cardiovascular disease patients, we recruited healthy participants who self-tracked health and physical activity data and attended a physical activity planning session with a healthcare professional (HCP). Subsequently both HCPs and participants were interviewed. In part two, findings from part one were presented to HCPs in a card-sorting workshop to corroborate findings and identify information needs of HCPs alongside patient journeys and clinical workflows. Our outcomes highlight HCP information needs around patient risk factors, vital signs, and adherence to physical activity. Enablers for PGHD integration include adaptive data sense-making, standardization and organizational support for integration. Barriers include lack of time, data quality, trust and liability concerns. Our research highlights implications for designing digital health technologies that support PGHD in physical activity planning during cardiac rehabilitation.

==> ALTtext.tex <==
Figure 1: Study Design Diagram: Diagram illustrating the 2-part study design process - Part 1) data collection by participants, consultations between HCPs and participants, follow up interviews with everyone. Part 2) Card sorting workshop

Figure 2: Healthcare Professional-Participant Consultations: Three photographs depicting individual consultations between healthcare professionals and healthy participants. Photo 1) A HCP is pointing his pen towards the self-tracking application on participant's mobile phone and explaining the data to the participant. Photo 2) A HCP is writing notes on the printed report, while participant browses through the mobile application. Photo 3) Participant shows his mobile phone to the HCP and points towards the screen while the HCP points his pen towards the application, while having a printed report in front of him.

Figure 3: Self-tracking Devices: Three photos of the Withings Scanwatch smartwatch, BPM connect blood pressure monitor and the Body Cardio weighing scale used in the study to collect participant data.

Figure 4: Card Sorting Workshop and Information Flow: A diagram illustrating the relationships between artifacts used in the card sorting workshop and how they present information to healthcare professionals (HCPs). Cards are categorized as Data, Time, Analytics, and Visualization. The figure includes a photograph of a sample card sorting arrangement and an example of the information presented to HCPs, showing the cards in no particular order: 
Card 1: context(where, when/when, why...)
Card 2: Steps
Card 3: Text (This card is handwritten)
Card 4: Week
Card 5: Bar Chart
Card 6: Find Extremum (with example description)
Objective: I want to know what the patient did when they had the highest and lowest step counts last week.

Figure 5: Barriers and Enablers for Implementation: A multilevel diagram presenting barriers (in red) and enablers (in green) to implementation, organized according to the NASSS (Nonadoption, Abandonment, Scale-up, Spread, and Sustainability) framework. The diagram identifies factors at the adopter, organizational, and wider system levels, such as barriers: distracting data, missing information about data quality, non-standard user interface, need for patient-HCP co interpretation, enablers: good usability, patient education on PGHD use, overview of data through printed reports, general factors: interoperability and integration, ethics and regulations.

Figure 6: Patient Information Needs Worksheet (Pre-Consultation): A photograph of a worksheet with various cards and handwritten descriptions detailing information needs recommended for patients to reflect on and prepare before physical activity planning consultations. The worksheet includes prompts for sleep quality information, heart rate changes over the day and throughout the week as line chart, steps per day and whether they are meeting targets as line chart.

Figure 7: HCP Information Needs Worksheet (Pre-Consultation): A photograph of a worksheet with various cards and handwritten descriptions detailing information needs recommended for healthcare professionals (HCPs) to prepare before physical activity planning consultations. The worksheet includes prompts for patient weight as line chart, contraindications and risks factors, blood pressure changes in morning compared to evening over the week bar chart.

Figure 8: Joint HCP-Patient Discussion Worksheet (During Consultation): A photograph of a worksheet with various cards and handwritten descriptions detailing information needs recommended for discussion between HCPs and patients during physical activity planning consultations. The worksheet covers topics such as a workflow to discuss 1) physical activity levels as bar chat, 2) blood pressure as line chart, 3) weight and body mass index  during weekdays as line chart, 4) sleep quality, 5) barriers and enablers and setting new goals as table (hand-drawn card). 

Figure 9: MoSCoW Prioritization of Data Points: A photograph of a worksheet with various cards detailing the MoSCoW (Must have, Should have, Could have, Won't have) prioritization of data points required for physical activity planning consultations. The cards categorize data points based on their importance for effective consultations. Must haves include heart rate, sedentary time, physical activity, MVPA level, steps and weight.

Figure 10: Prerequisites for Acceptable Digital Health Technologies (DHTs):
 A diagram illustrating a layered model approach outlining the prerequisites for successful digital health interventions. Overlapping arrows labeled "Accessibility," "Usability," and "Experience" point towards the concept of "Acceptable DHTs," suggesting these factors contribute to acceptability.
